A note on the expressive power of linear orders

This article shows that there exist two particular linear orders such that first-order logic with these two linear orders has the same expressive power as first-order logic with the Bit-predicate FO(Bit). As a corollary we obtain that there also exists a built-in permutation such that first-order logic with a linear order and this permutation is as expressive as FO(Bit).

==> Makros_Standard.tex <==
% file Makros_Standard.tex  17.01.2001
% letzte Aenderung: Nicole, 05.02.2003

\newcommand{\longpage}{\enlargethispage{\baselineskip}}
\newcommand{\shortpage}{\enlargethispage{-\baselineskip}}

\usepackage{url} % Damit kann man www-Adressen u.ae. richtig umbrechen
\usepackage{enumerate, stmaryrd,mathrsfs}
\usepackage{amsmath,amssymb,latexsym}
\usepackage{times} 
%\usepackage{pstricks,ifthen}


% neue Umgebung fuer ``enumerate'': ohne Absatz davor und danach
\newcounter{zaehler_enumerate_kurz}
\newenvironment{enumerate_kurz}
  { \begin{list}
      { (\alph{zaehler_enumerate_kurz}) 
      }
      { \usecounter{zaehler_enumerate_kurz} 
        \setlength{\topsep}{0pt} 
        \setlength{\parskip}{0pt}
        \setlength{\labelwidth}{4.5ex}
        \setlength{\leftmargin}{4.5ex}
        %\setlength{\labelsep}{1ex}
      }
  }
  { \end{list}
  }


%
%


% Abkuerzungen 
\newcommand*{\twodots}{.\,.\,}
\newcommand*{\twocdots}{{\cdot}\,{\cdot}\,}
\newcommand*{\ToDo}{{\textbf{ToDo!}}}

\newcommand*{\raus}[1]{ }

\newcommand*{\eg}{e.g.\ }
\newcommand*{\ie}{i.e.\ }


\newcommand*{\parno}{\par\noindent}
\newcommand*{\ov}[1]{\overline{#1}}
\newcommand*{\vek}[1]{\ensuremath{\vec{#1}}}
\newcommand*{\bigvek}[1]{\ensuremath{\overrightarrow{#1}}}

\newcommand*{\bs}[1]{\ensuremath{\boldsymbol{#1}}}



% logische Symbole: \exists, \forall, \models
\newcommand*{\und}{\ensuremath{\wedge}}
\newcommand*{\Und}{\ensuremath{\bigwedge}}
\newcommand*{\oder}{\ensuremath{\vee}}
\newcommand*{\Oder}{\ensuremath{\bigvee}}
\newcommand*{\nicht}{\ensuremath{\neg}}
\newcommand*{\impl}{\ensuremath{\rightarrow}}
\newcommand*{\gdw}{\ensuremath{\leftrightarrow}}

\newcommand*{\Qu}{\ensuremath{\mathsf{Q}}} % Q fuer Quantifier;
% z.B. um  \Qu\in\set{\exists,\forall} zu schreiben 


% math. Zeichen
\renewcommand*{\geq}{\ensuremath{\geqslant}}
\renewcommand*{\leq}{\ensuremath{\leqslant}}

\newcommand*{\set}[1]{\ensuremath{\{ #1 \}}}
\newcommand*{\setc}[2]{\set{#1 \,:\, #2}}

\newcommand*{\bigset}[1]{\ensuremath{ \left\{ #1 \right\} } }
\newcommand*{\bigsetc}[2]{\bigset{#1 \,:\, #2}}


\newcommand*{\DOM}[1]{\ensuremath{{[} #1 {]}}}
%\newcommand*{\dom}[1]{\ensuremath{\underline{#1}}}
\newcommand*{\dom}[1]{\ensuremath{[#1]}}


% INTERVALLE
\newcommand*{\interval}{\ensuremath{\textit{int\,}}}
\newcommand*{\cinterval}[1]{\ensuremath{\interval{[} #1 {]}}}
\newcommand*{\ointerval}[1]{\ensuremath{\interval{(} #1 {)}}}
\newcommand*{\cointerval}[1]{\ensuremath{\interval{[} #1 {)}}}
\newcommand*{\ocinterval}[1]{\ensuremath{\interval{(} #1 {]}}}
% bzw:
\newcommand*{\intoc}[1]{\ocinterval{#1}}
\newcommand*{\intco}[1]{\cointerval{#1}}
\newcommand*{\intcc}[1]{\cinterval{#1}}
\newcommand*{\intc}[1]{\cinterval{#1}}
\newcommand*{\intoo}[1]{\ointerval{#1}}
\newcommand*{\into}[1]{\ointerval{#1}}
% bzw:
\newcommand*{\intro}[1]{\intco{#1}}


%\newcommand*{\relational}{\ensuremath{\textit{rel}}}
\newcommand*{\relational}{\ensuremath{\textit{wofs}}} 
\newcommand*{\links}{\ensuremath{\scriptscriptstyle {-}}}
\newcommand*{\rechts}{\ensuremath{\scriptscriptstyle {+}}}

% mathematische Funktionen
\newcommand*{\FktsFont}[1]{\ensuremath{\textup{#1}}}

% lcm
\newcommand*{\lcm}{\ensuremath{\FktsFont{lcm}}}

\newcommand*{\abgerundet}[1]{\ensuremath{
    \left\lfloor {#1} \right\rfloor }}
\newcommand*{\aufgerundet}[1]{\ensuremath{\left\lceil {#1} \right\rceil }}
\newcommand*{\betrag}[1]{\ensuremath{\left| {#1} \right| }}

\newcommand*{\rep}{\ensuremath{\textit{rep}}}
%\newcommand*{\repcan}{\ensuremath{\textit{canrep}}}
\newcommand*{\repcan}{\ensuremath{\textit{rep}}}

\newcommand*{\Color}{\ensuremath{\textit{col\,}}}
\newcommand*{\ktype}{\ensuremath{k\textit{-type\,}}}

\newcommand*{\Char}{\ensuremath{\textit{char\,}}}




\newcommand*{\deff}{:=}
\newcommand*{\ffed}{=:}

\newcommand*{\modulo}[1]{\ensuremath{\ (\FktsFont{mod}\ #1)}}

%\newcommand*{\positive}{\mbox{\tiny $\scriptscriptstyle > 0$}}
\newcommand*{\NN}{\ensuremath{\mathbb{N}}}    % N f\"ur nat\"urliche
                                              % Zahlen  
\newcommand*{\NNpos}{\ensuremath{\NN_{\mbox{\tiny $\scriptscriptstyle > 0$}}}}

\newcommand*{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand*{\ZZpos}{\ensuremath{\ZZ_{\mbox{\tiny $\scriptscriptstyle > 0$}}}}
\newcommand*{\ZZneg}{\ensuremath{\ZZ_{\mbox{\tiny $\scriptscriptstyle < 0$}}}}

\newcommand*{\RR}{\ensuremath{\mathbb{R}}}
\newcommand*{\QQ}{\ensuremath{\mathbb{Q}}}
\newcommand*{\RRpos}{\ensuremath{\RR_{\mbox{\tiny $\scriptscriptstyle\geq 0$}}}}
\newcommand*{\UU}{\ensuremath{\mathbb{U}}}
\newcommand*{\VV}{\ensuremath{\mathbb{V}}}


\newcommand*{\A}{\ensuremath{\mathcal{A}}}
\newcommand*{\B}{\ensuremath{\mathcal{B}}}
\newcommand*{\C}{\ensuremath{\mathcal{C}}}
\newcommand*{\D}{\ensuremath{\mathcal{D}}}
\newcommand*{\Q}{\ensuremath{\mathcal{Q}}}

\newcommand*{\Abig}{\ensuremath{\mathfrak{A}}}
\newcommand*{\Bbig}{\ensuremath{\mathfrak{B}}}
\newcommand*{\Cbig}{\ensuremath{\mathfrak{C}}}
\newcommand*{\Dbig}{\ensuremath{\mathfrak{D}}}


\newcommand*{\abig}{\ensuremath{\mathfrak{a}}}
\newcommand*{\bbig}{\ensuremath{\mathfrak{b}}}
\newcommand*{\cbig}{\ensuremath{\mathfrak{c}}}
\newcommand*{\dbig}{\ensuremath{\mathfrak{d}}}
\newcommand*{\ubig}{\ensuremath{\mathfrak{u}}}
\newcommand*{\vbig}{\ensuremath{\mathfrak{v}}}

\newcommand*{\xbig}{\ensuremath{{x}}}
\newcommand*{\ybig}{\ensuremath{{y}}}
\newcommand*{\zbig}{\ensuremath{{z}}}

\newcommand*{\ablue}{\ensuremath{a_{\scriptscriptstyle\mathit{blue}}}}
\newcommand*{\bblue}{\ensuremath{b_{\scriptscriptstyle\mathit{blue}}}}

\newcommand*{\K}{\ensuremath{\mathscr{K}}}
\newcommand*{\Cl}{\ensuremath{\mathscr{C}}} % Cl fuer Class
\newcommand*{\Clfinite}{\ensuremath{\Cl_{\class{fin}}}}
\newcommand*{\Clfinrep}{\ensuremath{\Cl_{\class{fin.rep}}}}
\newcommand*{\Clarb}{\ensuremath{\Cl_{\class{arb}}}}
\newcommand*{\ClNrep}{\ensuremath{\Cl_{\class{$\NN$-rep}}}}
\newcommand*{\ClZrep}{\ensuremath{\Cl_{\class{$\ZZ$-rep}}}}
\newcommand*{\ClNemb}{\ensuremath{\Cl_{\class{$\NN$-emb}}}}
\newcommand*{\ClZemb}{\ensuremath{\Cl_{\class{$\ZZ$-emb}}}}

\newcommand*{\LL}{\ensuremath{\mathscr{L}}}

% Alphabet
%\newcommand*{\letter}[1]{\ensuremath{\texttt{\upshape #1}}} % fuer Buchstaben im Alphabet
\newcommand*{\letter}[1]{\ensuremath{\mathbb{#1}}} % fuer Buchstaben im Alphabet

\newcommand*{\Al}{\letter{A}} % fuer Alphabet A
\newcommand*{\AlB}{\letter{B}} % fuer Alphabet B

\newcommand*{\Qa}{\ensuremath{Q_{\letter{a}}}} % fuer Buchstaben-Praedikat Q_a
\newcommand*{\Qb}{\ensuremath{Q_{\letter{b}}}} 
\newcommand*{\Qe}{\ensuremath{Q_{\e}}} % fuer Buchstaben-Praedikat Q_e
\newcommand*{\QTrenn}{\ensuremath{Q_{\Trenn}}} % fuer Buchstaben-Praedikat Q_#
\newcommand*{\QNull}{\ensuremath{Q_{\letter{0}}}} % fuer Buchstaben-Praedikat Q_0
\newcommand*{\QEins}{\ensuremath{Q_{\letter{1}}}} % fuer Buchstaben-Praedikat Q_1
\newcommand*{\QbEins}{\ensuremath{Q_{\letter{b}_\letter{1}}}} 
\newcommand*{\Qbk}{\ensuremath{Q_{\letter{b}_{\letter{k}}}}} 


\newcommand*{\tauAl}{\ensuremath{\tau_{\Al}}} % fuer signature tau_Alphabet
\newcommand*{\tauAlB}{\ensuremath{\tau_{\AlB}}} 
\newcommand*{\tauAle}{\ensuremath{\tau_{\Al\cup\set{\e}}}}

\newcommand*{\tauOrdAdd}{\ensuremath{\tau_{\scriptscriptstyle <,+}}}

\newcommand*{\emptystring}{\ensuremath{\lambda}} % fuer empty string
\newcommand*{\e}{\ensuremath{\letter{e}}} % e fuer neutral letter
\newcommand*{\Trenn}{\ensuremath{\letter{\#}}} % Trennsymbol

\newcommand*{\OPair}[2]{\ensuremath{\textstyle {
      {\letter{#1}}\atop{\letter{#2}} }}} % 2 Buchstaben uebereinander; OHNE Klammern
\newcommand*{\Pair}[2]{\ensuremath{\textstyle {
      \left[{\letter{#1}}\atop{\letter{#2}}\right] }}} % 2 Buchstaben uebereinander; MIT Klammern
\newcommand*{\pair}[2]{\ensuremath{\textstyle {
      {{#1}}\atop{{#2}} }}} % 2 Zeichen uebereinander, OHNE Klammern, OHNE letter-style
                                          % 




\newcommand*{\U}{\ensuremath{\mathcal{U}}}
\newcommand*{\bigO}{\ensuremath{{\cal{O}}}}
%\newcommand*{\bigO}{\ensuremath{\mathcal{O}}}


%%%%%%%%%%%% Funktionen m(k), l(k), c(k), g(k)
\newfont{\MyScript}{cmfi10 at 10pt}
%\newcommand*{\mF}{\ensuremath{\mbox{\MyScript{m}}}}
%\newcommand*{\lF}{\ensuremath{\mbox{\MyScript{l}}}}
%\newcommand*{\cF}{\ensuremath{\mbox{\MyScript{c}}}}
%\newcommand*{\gF}{\ensuremath{\mbox{\MyScript{g}}}}
%\newcommand*{\rF}{\ensuremath{\mbox{\MyScript{r}}}}
\newcommand*{\mF}{\ensuremath{\mathtt{m}}}
\newcommand*{\lF}{\ensuremath{\mathtt{l}}}
\newcommand*{\cF}{\ensuremath{\mathtt{c}}}
\newcommand*{\gF}{\ensuremath{\mathtt{g}}}
\newcommand*{\rF}{\ensuremath{\mathtt{r}}}
%%%%%%%%%%%%

\newcommand*{\SC}{\ensuremath{\textit{SC}}}
\newcommand*{\SCd}{\ensuremath{\textit{SC'}}}
\newcommand*{\adom}{\ensuremath{\textsl{adom}}}
\newcommand*{\Cube}[1]{\ensuremath{\textit{Cube}_{#1}}}
\newcommand*{\Type}[1]{\ensuremath{\textit{Type}_{{#1}}}}
\newcommand*{\type}[1]{\ensuremath{\textit{type}_{{#1}}}}
\newcommand*{\types}{\ensuremath{\textbf{\itshape types}}}
\newcommand*{\Types}{\ensuremath{\textbf{\itshape Types}}}

\newcommand*{\dr}{\ensuremath{\textit{dr}}}
\newcommand*{\ar}{\ensuremath{\textit{ar}}}

\newcommand*{\diag}{\ensuremath{\textit{diag}}}



% Probleme
\newcommand*{\Problem}[1]{\ensuremath{\textsc{#1}}}

\newcommand*{\Spectrum}{\Problem{Spec}}

\newcommand*{\Parity}{\Problem{Parity}}

\newcommand*{\Reach}{\Problem{Reach}}
\newcommand*{\detReach}{\Problem{Det-Reach}}
\newcommand*{\Conn}{\Problem{Conn}}

%\newcommand*{\LImm}{\ensuremath{ L_{\textsl{\tiny Prop\,\ref{proposition:Immerman}}} }}
\newcommand*{\LImm}{\ensuremath{L_{\textup{Imm}}}}

\newcommand*{\BinLists}{\Problem{BinaryLists}}

\newcommand*{\Bin}{\ensuremath{\textit{BIN}}}
\newcommand*{\List}{\ensuremath{\textit{List\,}}}

\newcommand*{\Neutral}{\ensuremath{\textit{neutral\,}}}



% Strukturen
\newcommand*{\struc}[1]{\ensuremath{\big( #1 \big)}}
\newcommand*{\bigstruc}[1]{\ensuremath{
    \left( #1 \right)}}


%\newcommand*{\substruc}[2]{\ensuremath{#1\,{\downarrow}\,#2}}
\newcommand*{\substruc}[2]{\ensuremath{\langle #2 \rangle^{#1}}}


% Praedikate
\newcommand*{\praedikat}[1]{\ensuremath{\textsl{#1}}}
\newcommand*{\Bit}{\praedikat{Bit}}
\newcommand*{\Dy}{\praedikat{Dy}}
%\newcommand*{\Bit}{\ensuremath{\FktsFont{BIT}}}
\newcommand*{\Squares}{\praedikat{Squares}}
\newcommand*{\Primes}{\praedikat{Primes}}
\newcommand*{\Exp}{\praedikat{Exp}}
\newcommand*{\Inv}{\praedikat{Inv}}

\newcommand*{\Max}{\praedikat{max}}
\newcommand*{\Min}{\praedikat{min}}
\newcommand*{\Succ}{\praedikat{succ}}
\newcommand*{\SuccP}{\Succ^P}
\newcommand*{\Pred}{\praedikat{pred}}
\newcommand*{\PredP}{\Pred^P}


% Praedikatklasse
\newcommand*{\Praedikatklasse}[1]{\ensuremath{\mathfrak{#1}}}
\newcommand*{\Mon}{\Praedikatklasse{Mon}}
\newcommand*{\Arb}{\Praedikatklasse{Arb}}
\newcommand*{\Bip}{\Praedikatklasse{Bip}} % Bip fuer Built-In Predicates
\newcommand*{\Num}{\Bip} % Bip 
\newcommand*{\Rel}{\Bip} % Bip

\newcommand*{\Ord}{\Praedikatklasse{Ord}} % Ord fuer linear orderings

\newcommand*{\Groups}{\Praedikatklasse{Groups}}

\newcommand*{\Presb}{\Praedikatklasse{Presb}}
%\newcommand*{\Presb}{\ensuremath{\textit{Presb}}}



% Formeln
\newcommand*{\Log}{\ensuremath{\lg}}
\newcommand*{\Nr}{\#}
\newcommand*{\Count}{\#}
\newcommand*{\CountPF}{\#\textsl{PF}} % Anzahl der Primfaktoren

\newcommand*{\dwins}{\ensuremath{\approx}} % Duplicator has a winning strategy
\newcommand*{\dwinsBCEFO}{\ensuremath{\sim}} % Duplicator wins game for BCEFO
\newcommand*{\dwinsBCeFO}{\dwinsBCEFO} % andere Tipp-weise 

%\newcommand*{\entspricht}{\ensuremath{\hat{=}}}
\newcommand*{\entspricht}{\ensuremath{\stackrel{\und}{=}}}

\newcommand*{\form}[1]{\ensuremath{{\mathit{#1}}}}

\newcommand*{\free}{\ensuremath{\textit{free\,}}}

\newcommand*{\qd}{\ensuremath{\textit{qd\,}}}

\newcommand*{\VCdim}{\ensuremath{\textit{VC-dim\,}}}
\newcommand*{\Nx}{\ensuremath{n_{\vek{x}}}}
\newcommand*{\Ny}{\ensuremath{n_{\vek{y}}}}

\newcommand*{\block}{\form{block}}
\newcommand*{\num}{\form{num}}


% Formel- und Komplexitaetsklassen
\newcommand*{\class}[1]{\ensuremath{\textrm{\upshape{#1}}}}

\newcommand*{\FO}{\class{FO}}
\newcommand*{\FOunC}{\class{FOunC}}
\newcommand*{\FObinC}{\class{FObinC}}
\newcommand*{\FOkaryC}{\class{FO}k\class{-aryC}}
\newcommand*{\FOonearyC}{\class{FO}1\class{-aryC}}
\newcommand*{\FOtwoaryC}{\class{FO}2\class{-aryC}}

\newcommand*{\FOunM}{\class{FOunM}}
\newcommand*{\FObinM}{\class{FObinM}}

%%%%%%%%%%%
\newcommand*{\FOactive}{\FO_{\class{active}}}
\newcommand*{\OrderGen}{\ensuremath{{<}\class{-generic}\;}}
\newcommand*{\OrderGenFO}{\ensuremath{{<}\class{-generic}\;\FO}}
\newcommand*{\FOadom}{\FO_{\class{adom}}}

\newcommand*{\FOKleiner}{\ensuremath{\FOadom(<)}}
\newcommand*{\FONum}{\ensuremath{\FO(<,\Num)}}
\newcommand*{\FONumi}{\ensuremath{\FO(<,\allowbreak\Num')}}
\newcommand*{\FOMon}{\ensuremath{\FO(<,\Mon)}}
\newcommand*{\FOMoni}{\ensuremath{\FO(<,\Mon')}}
\newcommand*{\FOPlus}{\ensuremath{\FO(<,\allowbreak +)}}

\newcommand*{\BC}{\class{BC}}
\newcommand*{\EFO}{\class{EFO}}
\newcommand*{\BCeFO}{\ensuremath{\class{BC}(\EFO)}}
%\newcommand*{\BCeFO}{\class{BC(EFO)}}
\newcommand*{\BCeFOadom}{\BCeFO_{\class{adom}}}
\newcommand*{\BCeFOKleiner}{\ensuremath{\BCeFOadom(<)}}

\newcommand*{\BCEFO}[1]{\BCeFO(#1)}
%\newcommand*{\BCEFO}[1]{\class{BC}\big(\EFO(#1)\big)}

\newcommand*{\EFOmodsp}{\ensuremath{\Sigma_1^{(s,p)}}}
\newcommand*{\BCEFOmodsp}{\ensuremath{\class{BC}(\EFOmodsp)}}


%%%%%%%%%%%
\newcommand*{\LFP}{\class{LFP}}
\newcommand*{\GFP}{\class{GFP}}

\newcommand*{\TC}{\class{TC}}
\newcommand*{\DTC}{\class{DTC}}


\newcommand*{\Linf}{\ensuremath{{L}_{\infty\omega}^{\omega}}}
\newcommand*{\SO}{\class{SO}}
\newcommand*{\MSO}{\class{MSO}}

\newcommand*{\co}{\class{co}}
\newcommand*{\NP}{\class{NP}}
\newcommand*{\DP}{\class{P}}

\newcommand*{\ETIME}{\class{ETIME}}
\newcommand*{\LinH}{\class{LINH}}
\newcommand*{\Logspace}{\class{LOGSPACE}}
\newcommand*{\NLogspace}{\class{NLOGSPACE}}

\newcommand*{\TCzero}{\ensuremath{\class{TC}^0}}
\newcommand*{\ACzero}{\ensuremath{\class{AC}^0}}
\newcommand*{\ACO}{\ACzero}

\newcommand*{\Mod}{{\textsl{Mod}}}
\newcommand*{\MOD}{{\textsl{MOD}}}

%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Diss"
%%% End: 



